iFogSim: A Toolkit for Modeling and Simulation of Resource Management Techniques in Internet of Things, Edge and Fog Computing Environments

Internet of Things (IoT) aims to bring every object (e.g. smart cameras, wearable, environmental sensors, home appliances, and vehicles) online, hence generating massive amounts of data that can overwhelm storage systems and data analytics applications. Cloud computing offers services at the infrastructure level that can scale to IoT storage and processing requirements. However, there are applications such as health monitoring and emergency response that require low latency, and delay caused by transferring data to the cloud and then back to the application can seriously impact their performances. To overcome this limitation, Fog computing paradigm has been proposed, where cloud services are extended to the edge of the network to decrease the latency and network congestion. To realize the full potential of Fog and IoT paradigms for real-time analytics, several challenges need to be addressed. The first and most critical problem is designing resource management techniques that determine which modules of analytics applications are pushed to each edge device to minimize the latency and maximize the throughput. To this end, we need a evaluation platform that enables the quantification of performance of resource management policies on an IoT or Fog computing infrastructure in a repeatable manner. In this paper we propose a simulator, called iFogSim, to model IoT and Fog environments and measure the impact of resource management techniques in terms of latency, network congestion, energy consumption, and cost. We describe two case studies to demonstrate modeling of an IoT environment and comparison of resource management policies. Moreover, scalability of the simulation toolkit in terms of RAM consumption and execution time is verified under different circumstances.

==> Resources/tmp-pdfcrop-25051.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{6172636869746563747572652E706466}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{5}

